How Hard is this Test Set? NLI Characterization by Exploiting Training Dynamics

Natural Language Inference (NLI) evaluation is crucial for assessing language understanding models; however, popular datasets suffer from systematic spurious correlations that artificially inflate actual model performance. To address this, we propose a method for the automated creation of a challenging test set without relying on the manual construction of artificial and unrealistic examples. We categorize the test set of popular NLI datasets into three difficulty levels by leveraging methods that exploit training dynamics. This categorization significantly reduces spurious correlation measures, with examples labeled as having the highest difficulty showing markedly decreased performance and encompassing more realistic and diverse linguistic phenomena. When our characterization method is applied to the training set, models trained with only a fraction of the data achieve comparable performance to those trained on the full dataset, surpassing other dataset characterization techniques. Our research addresses limitations in NLI dataset construction, providing a more authentic evaluation of model performance with implications for diverse NLU applications.

==> sections.old/1.Introduction.tex <==
Natural Language Inference (NLI), or textual entailment \cite{dagan2009}, has emerged as an enduring challenge in the field of Natural Language Processing for evaluating the Natural Language Understanding (NLU) capabilities of models. Persistently, NLI remains a difficult problem, as it implies reasoning across several linguistic phenomena to determine the logical relationship (i.e., entailment, contradiction, and neutral) between two documents - a premise and a hypothesis. The capability to accurately infer relationships between sentences is crucial for a wide range of applications, such as question answering \cite{qanli}, dialogue systems \cite{welleck-etal-2019-dialogue}, and fact-checking \cite{9288228}. 

Since its inception \cite{nli-first}, several large-scale benchmark datasets have been proposed for NLI \cite{snli:emnlp2015,multi-nli,nie2019adversarial}; however, in time, the most ubiquitously used are the Stanford Natural Language Inference (SNLI) \cite{snli:emnlp2015} and the MultiNLI datasets \cite{multi-nli}, which have played a pivotal role in advancing the state of the art \cite{nlisurvey2019}.

However, multiple works \cite{liu2020hyponli,gururangan-etal-2018-annotation,tsuchiya-2018-performance,poliak-etal-2018-hypothesis,naik-etal-2018-stress,glockner-etal-2018-breaking} pointed out several critical limitations in these datasets, stemming from systematic annotation errors and spurious correlations that impact both the training and test sets. A critical consequence of these issues is the inflation of model performance, leading to seemingly high results \cite{naik-etal-2018-stress,liu2020hyponli} that may not generalize well to real-world scenarios. For example, a widely used RoBERTa model \cite{liu2019roberta} trained solely on the hypothesis achieves an unreasonable accuracy of XX\% on SNLI and YY\% on MultiNLI, which strongly points towards systematic errors in dataset construction.

In this work, we aim to address the limitations of existing NLI datasets by proposing an automated construction of a more challenging stress test. In contrast to previous approaches, we avoid manually creating artificial examples \cite{naik-etal-2018-stress}; instead, we leverage existing samples from the test set. We further generalize dataset cartography \cite{swayamdipta2020dataset} to cluster samples in the test set of each dataset and characterize them into three categories of increasing difficulty.

Our approach leverages training dynamics of each premise-hypothesis pair and is inspired by related works in both NLI \cite{naik-etal-2018-stress,geiger2018stress,liu2020hyponli} and approaches tackling the problem of learning with noisy data \cite{pleiss2020identifying}. We show that our method can isolate examples exhibiting spurious correlations and provide a challenging test set. Furthermore, our method is general, model-agnostic, and easily extensible to other datasets. Our experiments show that using the same method on the training set enables the aggressive filtering of uninformative examples during training, reducing data quantity but increasing quality, enabling the model to obtain on-par performance on the test set using only a fraction of data.

This work makes the following contributions:
\begin{enumerate}
    \item Denoting systematic annotation errors and spurious correlations in the test sets for two popular NLI datasets - SNLI \cite{snli:emnlp2015} and MultiNLI \cite{multi-nli}. We show statistically significant correlations between the performance of models and the presence of several measures of spurious correlations across labels.

    \item Proposing a general method for automatically characterizing examples in the test set into three increasing difficulty levels, which correlate with decreased model performance. Our method eliminates spurious correlations, providing a more accurate measure of model performance in the real world.

    \item The same procedure applied to the training data achieves similar performance on the test set while using only XX\% of the available data.
\end{enumerate}


==> sections.old/2.RelatedWork.tex <==
Across the development of natural language inference and understanding systems, multiple large-scale training and testing datasets have been developed across different linguistic domains. Initially, progress was driven by the addition of SNLI \cite{snli:emnlp2015}, but several other variants have been proposed, such as MultiNLI \cite{multi-nli}, containing multiple domains, SciNLI \cite{sadat-caragea-2022-scinli} and SciTail \cite{Khot2018SciTaiLAT} for scientific question answering, SQuAD \cite{rajpurkar-etal-2016-squad} and GLUE \cite{wang-etal-2018-glue} benchmarks for general-purpose NLU, and DOCNLI \cite{yin-etal-2021-docnli} containing long-form documents.

%%%%%%%%%%%%%%% Stress Tests
However, driven by the widespread observations that previous popular NLI datasets contain shortcuts \cite{tsuchiya-2018-performance,gururangan-etal-2018-annotation}, multiple works \cite{nie2019adversarial,glockner-etal-2018-breaking,naik-etal-2018-stress,geiger2018stress,yanaka2019help,saha2020conjnli} developed "stress tests" to benchmark specific linguistic and reasoning phenomena. 

\citet{glockner-etal-2018-breaking} proposed a simple test set based on SNLI \cite{snli:emnlp2015} that involves changing a single word in the premise sentences. In this setting, performance is substantially worse compared to the original SNLI test set, indicating the presence of spurious correlations in the training dataset construction.  \citet{naik-etal-2018-stress} proposed an NLI Stress Test by quantifying the lexical phenomena (e.g., presence of antonyms, numerical reasoning) behind common model errors in MultiNLI \cite{multi-nli}. Their proposed stress test involved constructing artificial examples that exacerbate common sources of model error, showcasing that some models have markedly reduced performance. \citet{nie2019adversarial} proposed a new benchmark called Adversarial NLI (ANLI), which leverages an interactive human-and-model-in-the-loop procedure to collect hard examples for natural language inference, obtaining a challenging stress test for current models. 

\citet{geiger2018stress} constructed a dataset of artificially built sentences based on first-order logic, fixing the sentence structure and only varying words corresponding to parts of speech at predefined positions. Such a dataset comprises unrealistic sentences but provides insight into the (lack-of) expressive power of certain neural architectures. Likewise, \citet{yanaka2019help} proposed the evaluation of monotonicity reasoning for NLI (i.e., inferences from subsets to supersets) by constructing a dataset through curating and manipulating sentence pairs from the Parallel Meaning Bank \cite{abzianidze-etal-2017-parallel}. \citet{saha2020conjnli} identified the lack of conjunctive reasoning examples in current NLI test sets and estimated that around 72\% of sentence pairs in SNLI have conjunctions unchanged between premise and hypothesis. The authors proposed CONJNLI, a stress test composed of conjunctive sentence pairs (i.e., containing conjunctions \textit{and}, \textit{or}) collected automatically from Wikipedia and manually verified. 

In contrast to previous work, we propose a method to characterize the test set into multiple difficulty levels by using training dynamics of neural networks \cite{swayamdipta2020dataset,pleiss2020identifying}, thereby isolating easy and spurious examples and keeping only challenging pairs. Our method is general, utilizes existing dataset samples (avoiding unrealistic artificial sentence pairs), is easily extensible to other datasets, and does not require manual verification of human annotators. Previous approaches \cite{naik-etal-2018-stress,saha2020conjnli} aim to develop a stress test for NLI by amplifying spurious correlations, evaluating model performance under various extreme conditions such as high presence of antonyms and word overlap, numerical reasoning, logical inferences and so on. In contrast, our goal is to minimize spurious correlations in existing benchmark datasets to gain a more realistic sense of performance under challenging real-world examples.

==> sections.old/3.Method.tex <==
\begin{figure*}[hbt!]
    % Diagram link: https://drive.google.com/file/d/1ku_CWosKI_udZjeawb4tF_S5spbOmgbI/view?usp=sharing
    \centering
    \includegraphics[width=1.0\textwidth]{figures/nli-diagram.drawio.png}
    \caption{Overall diagram of our method to automatically construct a challenging stress test for NLI. }
    \label{fig:diagram}
\end{figure*}

Our goal is to generalize the Data Maps proposed by \citet{swayamdipta2020dataset} to characterize the test set. \citet{swayamdipta2020dataset} proposed an approach to gauge the contribution of each training sample in a dataset by analyzing training dynamics (variability, average confidence of the gold label, and average correctness) across training for a fixed amount of epochs. After training, each example is split into one of three categories (i.e., \textit{easy-to-learn}, \textit{ambiguous} or \textit{hard-to-learn}) using a fixed percentile threshold on one of the features. For instance, instances regarded as \textit{ambiguous} are examples for which the variability across 5 epochs is in the top 33\% percentiles, disregarding other measures. 

We aim to extend and generalize Data Maps by employing a Gaussian Mixture Model \cite{Reynolds2009GaussianMM} to learn the best fitting distribution of data difficulty levels, thus avoiding fixed thresholds (e.g., using only 33\% of data). Figure \ref{fig:diagram} showcases the general methodology used in this work. We first characterize the test set by training two separate RoBERTa models with both premise and hypothesis (P+H), and hypothesis only (H); second, we gather 8 measures of training dynamics for each instance and cluster them to obtain three difficulty levels (4 for P+H and 4 for H). We found that difficulty levels simultaneously align with measures of spurious correlations and model performance.

In contrast to the initial approach of \citet{swayamdipta2020dataset}, we include 6 additional features for a more informative characterization across training. In our scenario focused on NLI in particular, we gather statistics for training dynamics across two types of settings: normal training (i.e., training with P + H) and hypothesis-only (H). Models trained only with the hypothesis have been shown to produce unreasonably high results \cite{poliak-etal-2018-hypothesis,liu2020hyponli}, mostly due to artifacts in dataset construction. These insights enabled us to gather statistics about such examples and improve data characterization through more complete and diverse features for each instance.

\input{algorithms/the-algorithm}

Different from \citet{swayamdipta2020dataset} who focused on characterizing the training set for increasing data quality, we aim to construct automatically a more challenging test set. A high-level overview of our method is presented in Algorithm \ref{alg:test-set-construction}. As such, in order to construct a data map of the test set, we trained a RoBERTa \cite{liu2019roberta} model for $E = 5$ epochs on the \textit{test set} using premise and hypothesis and, separately, using only the hypothesis. Let $D_{test} = \{(x, y^*)_i\}^N_{i = 1}$ be a test dataset containing $N$ instances, where, in our case, $x_i$ is comprised of a premise + hypothesis pair or only a hypothesis. We compute the following measures across training a RoBERTa model in both scenarios (P + H and H) for each example $x_i$: confidence ($\hat{\mu}_i$), variability ($\hat{\sigma}_i$), correctness ($\hat{c}_i$) and Area Under Margin (AUM; ${\textnormal{\textit{AUM}}}_i$). 

\begin{equation}
    \hat{\mu}_i = \frac{1}{E} \sum^{E}_{e = 1}p_{\boldsymbol{\theta}^{(e)}}(y^*_i | \boldsymbol{x_{i}})
    \label{eq:confidence}
\end{equation}

\begin{equation}
    \hat{\sigma}_i = \sqrt{\frac{\sum^{E}_{e = 1}(p_{\boldsymbol{\theta}^{(e)}}(y^*_i | \boldsymbol{x_{i}}) - \hat{\mu}_i)}{E}}
    \label{eq:variability}
\end{equation}

\begin{equation}
    \hat{c}_i = \frac{1}{E} \sum^{E}_{e = 1} [\operatorname*{argmax}(p_{\boldsymbol{\theta}^{(e)}}(x_i)) = y^*_i]
    \label{eq:corectness}
\end{equation}

where $p_{\boldsymbol{\theta}^{(e)}}$ corresponds to the model's probability during training at epoch $e$. Following \cite{swayamdipta2020dataset}, we compute confidence, variability, and correctness concerning the correct label $y^*_i$. Furthermore, we compute AUM \cite{pleiss2020identifying}, initially proposed as a method to identify mislabeled examples but yielding similar characterizations as Data Maps. We include AUM as an additional measure of instance correctness/learnability. Let $z^{(e)}_y (x_i)$ be the logit (pre-softmax) for class $y$ of the model at epoch $e$, given an instance $x_i$. The area under margin (AUM or average margin) of $x_i$ is computed as:

\begin{equation}
    {\textnormal{\textit{AUM}}}_i = \frac{1}{E} \sum^{E}_{e = 1} (z^{(e)}_{y^*_i}(x_i) - \operatorname*{max}_{(y \neq y^*_i)} z^{(e)}_y (x_i))
    \label{eq:AUM}
\end{equation}

Training the pretrained RoBERTa models for dataset characterization was performed for 5 epochs each, with a batch size of 32, using the Adam \cite{KingBa15} optimizer with a learning rate of $10^{-5}$ following a linear decay schedule with warm-up. We used mixed precision for all training runs. Training was performed on two NVIDIA RTX 2070 GPUs with 8GB of VRAM each. In Table \ref{tab:roberta-results}, we show the results of our RoBERTa models trained on SNLI and MultiNLI on different configurations of training/testing splits and using both the premise and the hypothesis or only the hypothesis. Our reproduction of results is on par with other works. For completeness, we also show results where the model is trained on the test set, but note that the purpose is only to gather training dynamics. The model trained on only the hypothesis obtains 71\% accuracy on SNLI and 61\% accuracy on MultiNLI, while random chance performance is 33\%. These results strongly point toward spurious correlations and annotation artifacts on both datasets \cite{tsuchiya-2018-performance,gururangan-etal-2018-annotation,poliak-etal-2018-hypothesis,liu2020hyponli}. 

\input{tables/roberta-results}

After training two RoBERTa models (P + H and H) on each dataset's test set, we construct a feature vector $f_i$ describing the training dynamics of an instance $i$ by concatenating the training dynamics of each sample in both settings:

\begin{equation}
    \begin{split}
    f^{(P+H)}_i &= [\hat{\mu}^{(P + H)}_i, \hat{\sigma}^{(P + H)}_i, \hat{c}^{(P + H)}_i, {\textnormal{\textit{AUM}}}^{(P + H)}_i] \\
    f^{(H)}_i &= [\hat{\mu}^{(H)}_i, \hat{\sigma}^{(H)}_i, \hat{c}^{(H)}_i, {\textnormal{\textit{AUM}}}^{(H)}_i] \\
    f_i &= f^{(P+H)}_i \mathbin\Vert f^{(H)}_i
    \end{split}
    \label{eq:features}
\end{equation}

\begin{figure*}[hbt!]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/snli_features_hardness.png}
    \includegraphics[width=1.0\textwidth]{figures/multi_nli_features_hardness.png}
    \caption{Distributions of feature values across difficulty levels for the test set for SNLI (top) and MultiNLI (bottom). In addition to features explored in Data Maps \cite{swayamdipta2020dataset}, we also incorporated the Average Margin \cite{pleiss2020identifying} and included training dynamics across a model trained only on the hypothesis.}
    \label{fig:snli-mnli-features}
\end{figure*}

Using the feature vectors $\{f_i\}^{N}_{i=1}$, we cluster the test set using a Gaussian Mixture Model into three clusters. Feature vectors are normalized with standard scaling. The clusters are ranked according to the intra-cluster average confidence $\hat{\mu}^{(P + H)}$, and we interpret them as belonging to three difficulty levels, following the terminology introduced by \citet{swayamdipta2020dataset}: \textit{easy}, \textit{ambiguous} and \textit{hard} (in decreasing order of $\hat{\mu}^{(P + H)}$). 

Figure \ref{fig:snli-mnli-features} depicts the distribution of features across difficulty levels for both datasets. While each type of feature captures different aspects of the learnability of an instance, their combination offers a more complete view of the learning dynamics during training. In the case of both SNLI and MultiNLI, harder examples have consistently lower average confidence and more variability of the correct class. The effect is not as pronounced in a hypothesis-only setting; however, there is a clear delimitation of easy examples for average margin and confidence, indicating potential annotation artifacts. 

Table \ref{tab:accuracy-per-split} shows the performance of a RoBERTa model trained on each dataset's training set and evaluated on our stress test after characterization using training dynamics. Easier instances have more examples annotated with contradiction and entailment, while harder instances have more examples annotated with "neutral". Performance monotonously degrades upon increasing the difficulty levels, reaching 56\% accuracy on SNLI-hard and 0.53\% accuracy on MultiNLI-hard. Performance on the easy split for both datasets is considerably higher compared to the global accuracy with all splits combined. Furthermore, the accuracy of a model trained using only the hypothesis degrades to almost random chance on harder splits, indicating that the hard split has fewer annotation artifacts. Compared to \citet{swayamdipta2020dataset}, the difficulty levels are not equal in size; the majority ($\sim$70\%) of samples belongs to the easy category, while only around 10\% are characterized as being hard. 

\input{tables/accuracy-per-split}

\begin{figure}[hbt!]
    \centering
    \includegraphics[width=0.90\linewidth]{figures/hardness-counts.png}
    \caption{Counts for each class in both SNLI and MultiNLI, according to each difficulty level.}
    \label{fig:hardness-counts}
\end{figure}

\input{tables/heuristics-definition}

\input{tables/qualitative-examples}

\begin{figure*}[hbt!]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/snli_heuristics.png}
    \includegraphics[width=1.0\linewidth]{figures/multi_nli_heuristics.png}
    \caption{Distributions of the measures of spurious correlations for each difficulty level (\textit{easy}, \textit{ambiguous}, \textit{hard}) across the three labels (\textit{entailment}, \textit{neutral}, \textit{contradiction}) for SNLI (top) and MultiNLI (bottom).}
    \label{fig:stats-heuristics}
\end{figure*}

Even though the hard split is relatively small, the subsample is challenging for current models, as it is comprised of instances where there are fewer spurious correlations between premise and hypothesis. Fewer annotation artifacts enable correct predictions from linguistic patterns in the hypothesis. In Figure \ref{fig:hardness-counts}, we show per-class counts relative to the difficulty levels for both datasets. It is the case that easier samples contain more contradictions and entailments, which are prone to have linguistic commonalities (word overlap, presence of antonyms). Consequently, the "hard" split has more neutral instances. In Table \ref{tab:qualitative-examples}, we showcase selected samples from each difficulty level. Through manual inspection, we found that for SNLI, the easy splits contain unrelated sentences which are sometimes annotated incorrectly as "Contradiction" (e.g., "a woman running in the park" versus "a man cooking at home" - two unrelated sentences annotated as contradicting).  For MultiNLI, we found that the easy split usually aligns with simple sentence negations (e.g., "it gets it" versus "it doesn't get it") or paraphrasing ("I guess history repeats itself" versus "history certainly doesn't repeat"). These observations strongly point towards spurious correlations between premise and hypothesis, making the sentences easier to correctly classify. The hard splits in both datasets contain more subtle cues, with little overlap in words between premise and hypothesis (e.g., "enjoying" a game versus just "playing" / "artists install a new exhibit" versus "people put up new art"), having more natural and challenging sentence pairs.

In the interest of quantifying the number of spurious correlations found in the test set, we follow \citet{naik-etal-2018-stress} and track several measures that correspond to either shallow statistics between the premise and the hypothesis such as word overlap, number of antonyms, or length mismatch, or the presence of negations or misspelled words. Table \ref{tab:heuristics} presents the heuristics implemented in our work. We automatically compute each measure, avoiding time-consuming manual annotations.

Across both SNLI and MultiNLI, we tracked the average amount of each measure between difficulty levels and classes (Figure \ref{fig:stats-heuristics}). To rigorously test the difference between the classes at various difficulty levels, we perform a non-parametric two-sided Mann-Whitney-U test \cite{mann1947test} with Bonferroni correction to test for statistical significant differences\footnote{Significance thresholds: Not Significant (ns): $p \leq 1.0$, *: $0.01 \le p \leq 0.05$, **: $0.001 \le p \leq 0.01$, ***: $0.0001 \le p \leq 0.001$, ****: $p \leq 0.001$}. The amount of spurious correlation is significantly reduced (Mann-Whitney's U test $p > 0.05$) in the hard split between the three classes. Some measures are more associated with certain classes. For instance, instances annotated with contradiction have a disproportionate amount of antonyms between premise and hypothesis in the easy and ambiguous splits. Similarly, negation is more present in the contradiction class for easy splits. For instances annotated with entailment, word overlap is present significantly in easy splits. For both SNLI and MultiNLI, our method yields little to no significant differences between classes in the hard split across the spurious correlation measures.

==> sections.old/4.ExperimentsResults.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Our method provides a more challenging test set, devoid of shortcuts and spurious correlations. However, we explore the possibility of using this approach to also improve data quality for training NLI models. To this end, we employ the same algorithm to characterize the training sets for SNLI and MultiNLI and train a RoBERTa model on different combinations of difficulty levels. Under each configuration, the RoBERTa model is trained for 10 epochs with early stopping on the validation set loss, with a learning rate of $10^{-5}$ following a linear decay schedule with a warm-up. 

We evaluate each model on both our stress test and the stress test proposed by \citet{naik-etal-2018-stress} that is based on MultiNLI. However, we emphasize that while the stress test of \citet{naik-etal-2018-stress} is designed to unrealistically amplify spurious correlations to gauge the model performance under various extreme conditions, our method eliminates linguistic shortcuts while mimicking real-world examples.

In Tables \ref{tab:our-snli-stress-test-results} and \ref{tab:our-multinli-stress-test-results}, we showcase results on SNLI and MultiNLI, respectively, in comparison with other training set characterization methods. In particular, we compare with Data Maps \cite{swayamdipta2020dataset} and Area Under Margin \cite{pleiss2020identifying}, two popular methods for training set characterizations using training dynamics. For Data Maps, we select ambiguous examples by keeping the instances where average variability is in the top 66\% percentile. For AUM, while the authors did not explicitly propose a threshold for characterizing each instance, we follow a similar approach to Data Maps, by considering ambiguous examples to have an average margin between the 33\% and 66\% percentiles.

\input{tables/snli_their_stress_test}
\input{tables/multinli_their_stress-test}

\input{tables/snli-stress-test-results}
\input{tables/multinli-stress-test-results}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

{\color{red} TODO comment on  Tables \ref{tab:our-snli-stress-test-results} and \ref{tab:our-multinli-stress-test-results}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In Tables \ref{tab:snli-their-stress-test-results} and \ref{tab:multinli-their-stress-test-results} we showcase performance on the dataset proposed by \citet{naik-etal-2018-stress} for RoBERTa models trained on SNLI and MultiNLI, respectively. The authors provided metadata for each instance in their stress test that allows fine-grained evaluation under different linguistic reasoning phenomena.

{\color{red} TODO comment on Tables \ref{tab:snli-their-stress-test-results} and \ref{tab:multinli-their-stress-test-results}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections.old/5.Conclusions.tex <==
In conclusion, our method highlights significant shortcomings in widely used NLI evaluation datasets (i.e., SNLI and MultiNLI) due to systematic annotation errors and spurious correlations. To address these issues, we proposed an automatic method for constructing more challenging test sets, effectively filtering out problematic instances and providing a more realistic measure of model performance. Our approach, which categorizes examples based on increasing difficulty levels, enhances evaluation reliability and offers insights into underlying challenges in NLI. Importantly, our methodology is versatile and can be applied across different datasets and models, promising improved evaluation practices in NLP.

By aggressively filtering uninformative examples, we show that comparable model performance can be achieved with significantly reduced data requirements. Overall, our work contributes to advancing NLI evaluation standards, fostering the development of more robust and generalizable NLU models capable of real-world applications.

==> tables/annotated-performance.tex <==
\begin{table*}[hbt!]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|ccc|ccc|ccc}
         & \multicolumn{3}{c}{\textbf{Entailment}} & \multicolumn{3}{c}{\textbf{Neutral}} & \multicolumn{3}{c}{\textbf{Contradiction}} \\
        & \textbf{Easy} & \textbf{Ambiguous} & \textbf{Hard} & \textbf{Easy} & \textbf{Ambiguous} & \textbf{Hard} & \textbf{Easy} & \textbf{Ambiguous} & \textbf{Hard} \\
        \toprule
        \textbf{SNLI - Incorrectly Labeled} & 0.23 & 0.27 & 0.39 & 0.03 & 0.13 & 0.43 & 0.69 & 0.61 & 0.36\\
        \textbf{SNLI - Accuracy} & 0.77 (0.99) & 0.69 (0.95) & 0.33 (0.41) & 
                        0.99 (0.98) & 0.95 (0.87) & 0.99 (0.57) & 
                        0.3 (0.99) & 0.31 (0.92) & 0.26 (0.55) \\ 
        \midrule
        \textbf{MultiNLI - Incorrectly Labeled} & 0.23 & 0.27 & 0.39 & 0.03 & 0.13 & 0.43 & 0.69 & 0.61 & 0.36\\
        \textbf{MultiNLI - Accuracy} & 0.77 (0.99) & 0.69 (0.95) & 0.33 (0.41) & 
                        0.99 (0.98) & 0.95 (0.87) & 0.99 (0.57) & 
                        0.3 (0.99) & 0.31 (0.92) & 0.26 (0.55) \\ 
    \end{tabular}
    }
    \caption{Model accuracy based on our verification annotations.}
    \label{tab:our-annotated_performance}
\end{table*}

==> tables/multinli-stress-test-results.tex <==
\begin{table}[hbt!]
    \centering
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{p{3.9cm}l|cccc}
        & & \multicolumn{4}{c}{\textbf{Our MultiNLI Stress Test}}\\
        \textbf{MultiNLI Diff. Splits} & \textbf{\% Data} & \textbf{Easy} & \textbf{Ambiguous} &  \textbf{Hard} & \textbf{Overall}\\
        \toprule
        AUM - Ambiguous \cite{pleiss2020identifying} & 33\% & 0.947 & 0.6415 & 0.4359 & 0.8500\\
        Data Maps - Ambiguous \cite{swayamdipta2020dataset} & 33\% & 0.9148 & 0.7085 & 0.4359 & 0.8355 \\
        \midrule
        % Random Subset & 45\% & 0.9526 & 0.7194 & 0.4493 & 0.8669\\
        Random Subset & 33\% & 0.9477 & 0.7154 & 0.4546 & 0.8631\\
        \midrule
        Easy & 41\% & 0.9500 &  0.6183 &  0.3994 & 0.8451 \\
        Easy - Ambiguous & 84\% &  0.9519 &  0.7366 &  0.4813 & 0.8721 \\
        Ambiguous & 43\% & 0.9516 &  0.7077 &  0.4813 & 0.8678 \\
        Ambiguous - Hard & 59\% & 0.9465 & 0.7451 & 0.4921 & 0.8704 \\
        Easy - Hard & 56\% & 0.9404 & 0.6549 & 0.4339 & 0.8468 \\
        Hard & 15\% & 0.4764 &  0.5704 & 0.284 & 0.4701\\
        \midrule
        Full Dataset & 100\% & 0.9470 & 0.7577 & 0.5374 & 0.8773 \\
    \end{tabular}
    }
    \caption{Results of a RoBERTa model trained on MultiNLI in various difficulty configurations and evaluated on our characterized MultiNLI stress test. The model achieves comparable performance using only a fraction of data.}
    \label{tab:our-multinli-stress-test-results}
\end{table}

==> tables/snli-stress-test-results.tex <==
\begin{table}[hbt!]
    \centering
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{p{4cm}l|cccc}
        & & \multicolumn{4}{c}{\textbf{Our SNLI Stress Test}}\\
        \textbf{SNLI Diff. Splits} & \textbf{\% Data} & \textbf{Easy} & \textbf{Ambiguous} &  \textbf{Hard} & \textbf{Overall}\\
        \toprule
        AUM - Ambiguous \cite{pleiss2020identifying} & 33\% & 0.9784 & 0.8736 & 0.4545 & 0.8955\\
        Data Maps - Ambiguous \cite{swayamdipta2020dataset} & 33\% & 0.9575 & 0.8551 & 0.5074 & 0.8841\\
        \midrule
        % Random Subset & 45\% & 0.9799 & 0.8765 & 0.5179 & 0.9048\\
        Random Subset & 33\% & 0.9786 & 0.8771 & 0.5008 & 0.9019\\
        \midrule
        Easy & 53\% & 0.9794 &  0.8371 &  0.4025 & 0.8833 \\
        Easy - Ambiguous & 86\% &  0.9819 &  0.887 &  0.5149 & 0.9077 \\
        Ambiguous & 33\% & 0.9805 &  0.8841 &  0.5099 & 0.9056 \\
        Ambiguous - Hard & 46\% & 0.9673 &   0.8736 &  0.5140 & 0.8951 \\
        Easy - Hard & 66\% & 0.9771 &  0.8441 &  0.4843 & 0.8930\\
        Hard & 13\% &  0.2922 & 0.3536 & 0.4909 & 0.3275\\
        \midrule
        Full Dataset & 100\% & 0.9779 & 0.8915 & 0.5677 & 0.9122 \\
    \end{tabular}
    }
    \caption{Results of a RoBERTa model trained on SNLI in various difficulty configurations and evaluated on our characterized SNLI stress test. The model achieves comparable performance using only a fraction of data.}
    \label{tab:our-snli-stress-test-results}
\end{table}

==> tables/theirs-compressed.tex <==
\begin{table*}[hbt!]
    \renewcommand\thetable{2}
    \begin{floatrow}

    \ttabbox{%
       \caption{Results for a RoBERTa model trained on SNLI in various configurations and evaluated on the stress test by \citet{naik-etal-2018-stress} based on MultiNLI. Best results across characterizations are \textbf{bold} and second best are \underline{underlined}.}
%
    }{%
     \begin{adjustbox}{width=0.5\textwidth}
        \begin{tabular}{lll|p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}cc}
            & & \multicolumn{7}{c}{\textbf{Stress Test by \citet{naik-etal-2018-stress}}}\\
            \textbf{Method} & \textbf{Splits} & \textbf{\% SNLI} &  \textbf{Word} \newline \textbf{Overlap} & \textbf{Spelling} \newline \textbf{Error} & \textbf{Numerical} \newline \textbf{Reasoning} &  \textbf{Negation} & \textbf{Length} \newline \textbf{Mismatch} & \textbf{Antonym} & \textbf{Overall} \\
            \toprule
            Data Maps  & Amb.  & 33\% & 0.6792 & 0.7202 & 0.3745 & 0.5388 & 0.7176 & 0.6237 & 0.6662\\
            AUM & Amb.  & 33\% & 0.6818 & 0.6904 & 0.2896 & 0.4837 & 0.7134 & \textbf{0.7417} & 0.6416\\
            \midrule
            % Random Subset & 45\% & 0.7187 & 0.7362 & 0.3889 & 0.6248 & 0.7546 & 0.6881 & 0.6998\\
            % Random Subset & 33\% & 0.7104 & 0.7277 & 0.3555 & 0.6009 & 0.7424 & 0.6312 & 0.6860\\
            % \midrule
            \multirow{6}{*}{\textbf{Ours}} & Easy                & 53\%  & 0.6720 &       0.6713 &            \underline{0.4287} &  0.4622 &        0.6870 &  0.4446 & 0.6246 \\
            & Easy - Amb.    & 86\%  & 0.7231 &        \textbf{0.7500} &            \textbf{0.4452} &  \underline{0.6124} &        \textbf{0.7578} &  0.6582 & \underline{0.7083} \\
            & Amb.           & 33\%  & \underline{0.7264} &       \underline{0.7414} &            0.4158 &  \textbf{0.6666} &        \underline{0.7491} &  0.6515 & \textbf{0.7093} \\
            & Amb. - Hard    & 46\%  & \textbf{0.7302} &        0.7305 &            0.3761 &  0.5533 &        0.7471 &  \underline{0.6619} & 0.6860\\
            & Easy - Hard         & 66\%  & 0.6714 &       0.6815 &            0.3803 &  0.5617 &        0.6993 &  0.4971 & 0.6442\\
            & Hard                & 13\%  & 0.3191 &       0.3310 &            0.3304 &  0.3184 &        0.3189 &     0.0 & 0.3177\\
            \midrule
            & Full Dataset        & 100\% & 0.7252 & 0.7559 & 0.2794 & 0.5923 & 0.7771 & 0.7268 & 0.7037\\
        \end{tabular}
    \end{adjustbox}
    \label{tab:snli-their-stress-test-results}
}
    \renewcommand\thetable{4}
    \ttabbox{%
    \caption{Results for a RoBERTa model trained on MultiNLI in various configurations and evaluated on the stress test proposed by \citet{naik-etal-2018-stress} based on MultiNLI. Best results across characterizations are \textbf{bold} and second best are \underline{underlined}.}
    %
    }{%
     \begin{adjustbox}{width=0.5\textwidth}
        \begin{tabular}{p{1.5cm}ll|p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}cc}
        & & \multicolumn{6}{c}{\textbf{Stress Test by \citet{naik-etal-2018-stress}}}\\
        \textbf{Method} & \textbf{Splits} & \textbf{\% MultiNLI} & \textbf{Word} \newline \textbf{Overlap} & \textbf{Spelling} \newline \textbf{Error} & \textbf{Numerical} \newline \textbf{Reasoning} &  \textbf{Negation} & \textbf{Length} \newline \textbf{Mismatch} & \textbf{Antonym} & \textbf{Overall} \\
        \toprule
        DataMaps & Amb.    & 33\% & \underline{0.7046} & 0.7938 & 0.4065 & 0.5469 & 0.8197 & 0.5712 & 0.7222\\
        AUM & Amb.          & 33\% & 0.6428 & 0.7998 & 0.2888 & \underline{0.5638} & 0.8254 & 0.5129 & 0.7115\\
        \midrule
        % Random Subset & 45\% & 0.7275 & 0.8216 & 0.4410 & 0.5811 & 0.8403 & 0.5834 & 0.7492\\
        % Random Subset & 33\% & 0.7408 & 0.8118 & 0.4331 & 0.5846 & 0.8321 & 0.5942 & 0.7455\\
        % \midrule
        \multirow{6}{*}{\textbf{Ours}} & Easy & 41\% & 0.6885 &       0.7978 &  0.3391 &  0.5514 &        0.8210 &  0.5274 & 0.7179\\
        & Easy - Amb.   & 84\% & 0.6601 &       \underline{0.8274} &            \textbf{0.4777} &  \textbf{0.5764} &        \underline{0.8467} &  \textbf{0.6330} & \underline{0.7459} \\
        & Amb.          & 43\% &  0.6283 &       0.8235 &            0.4602 &  0.5578 &        0.8421 &  0.5742 & 0.7337 \\
        & Amb. - Hard   & 59\% & 0.6961 &       \textbf{0.8255} &            \underline{0.4651} &  0.5628 &         \textbf{0.8476} &  \underline{0.6288} & \textbf{0.7474} \\
        & Easy - Hard   & 56\% & \textbf{0.7170} &       0.8032 &            0.2948 &  0.5607 &        0.8258 &  0.5062 & 0.7237\\
        & Hard & 15\%   & 0.4525 &       0.4966 &            0.2705 &  0.4589 &        0.4914 &  0.2506 &   0.4656 \\
        \midrule
        & Full Dataset & 100\% & 0.6701 & 0.8308 & 0.5380 & 0.5654 & 0.8500 & 0.6312 & 0.7511\\
    \end{tabular}
    \end{adjustbox}
    \label{tab:multinli-their-stress-test-results}
    }

\end{floatrow}
\end{table*}


